Real-Time Streaming and Event-driven Control of Scientific Experiments

Advancements in scientific instrument sensors and connected devices provide unprecedented insight into ongoing experiments and present new opportunities for control, optimization, and steering. However, the diversity of sensors and heterogeneity of their data result in make it challenging to fully realize these new opportunities. Organizing and synthesizing diverse data streams in near-real-time requires both rich automation and Machine Learning (ML). To efficiently utilize ML during an experiment, the entire ML lifecycle must be addressed, including refining experiment configurations, retraining models, and applying decisions-tasks that require an equally diverse array of computational resources spanning centralized HPC to the accelerators at the edge. Here we present the Manufacturing Data and Machine Learning platform (MDML). The MDML is designed to standardize the research and operational environment for advanced data analytics and ML-enabled automated process optimization by providing the cyberinfrastructure to integrate sensor data streams and AI in cyber-physical systems for in-situ analysis. To achieve this, the MDML provides a fabric to receive and aggregate IoT data and simultaneously orchestrate remote computation across the computing continuum. In this paper we describe the MDML and show how it is used in advanced manufacturing to act on IoT data and orchestrate distributed ML to guide experiments.

==> design.tex <==
\section{Design}

The design of the MDML platform is motivated by the unique needs 
and challenging demands of next-generation and scale-up research and development. The
MDML is designed to enable scientists to dynamically
integrate scientific IoT device data during high throughput experiments. 
To achieve these goals the MDML must standardize interfaces to facilitate 
plug-and-play integration of new sensors, provide intuitive management and 
extensible visualization capabilities, and incorporate the heterogeneous compute 
and data fabrics available in research laboratories. Here we outline how the MDML is designed to accommodate these goals. 

The MDML is composed of three layers: a \emph{data layer}, a {management and orchestration layer}, and \emph{visualization layer}


\subsection{Data Layer}

Providing software developers and scientists easy and intuitive mechanisms to integrate their instruments and IoT devices into the MDML. To achieve this goal we focus on reducing the barriers to connecting a device with the MDML.


Data interface -- data streamed in.

Data storage -- time series databases


\subsection{Management and Orchestration Layer}

\subsubsection{Data management}

\subsubsection{Distributed analysis}

A key requirement of the MDML platform is to incorporate and leverage the entire computing continuum, including edge devices co-located with an instrument and 
laboratory servers, through to HPC clusters and the cloud. To facilitate this remote, distributed computing model the MDML must leverage
tools to interface with
diverse computing resources while providing tools to seamlessly transmit data and codes for execution. Further, strict authorization and authentication policies must be followed to securely enable this federated computing model.



\subsection{Visualization Layer}
A key goal of the MDML is to remove barriers to accessing advanced insight into the ongoing state of an experiment. To achieve this we focus on two key areas: simplifying the integration and management of new data sources, and providing custom interfaces to visualize the state of an experiment.

The MDML provides capabilities for users to organize, annotate, and collate both their data sources and data sets. 

Further, the MDML provides extensible visualization capabilities to 
allow users to create custom portals to monitor experiments. These interfaces
are automatically populated by the MDML as data are collected and analyses are performed. Users can customize their portals to meet the needs of their 
experiment.

\ryan{Websites?}

